A Comprehensive Review of the Video-to-Text Problem

Research in the Vision and Language area encompasses challenging topics that seek to connect visual and textual information. When the visual information is related to videos, this takes us into Video-Text Research, which includes several challenging tasks such as video question answering, video summarization with natural language, and video-to-text and text-to-video conversion. This paper reviews the video-to-text problem, in which the goal is to associate an input video with its textual description. This association can be mainly made by retrieving the most relevant descriptions from a corpus or generating a new one given a context video. These two ways represent essential tasks for Computer Vision and Natural Language Processing communities, called text retrieval from video task and video captioning/description task. These two tasks are substantially more complex than predicting or retrieving a single sentence from an image. The spatiotemporal information present in videos introduces diversity and complexity regarding the visual content and the structure of associated language descriptions. This review categorizes and describes the state-of-the-art techniques for the video-to-text problem. It covers the main video-to-text methods and the ways to evaluate their performance. We analyze twenty-six benchmark datasets, showing their drawbacks and strengths for the problem requirements. We also show the progress that researchers have made on each dataset, we cover the challenges in the field, and we discuss future research directions.

==> sections/evaluation.tex <==
\section{Evaluation Measures}\label{sec:metrics}

As we have exposed before, the VTT problem can be mainly addressed by two types of methods: matching \& ranking-based techniques or NLG-based techniques.
Although the way to evaluate the results in both categories is not the same, the metrics used in both cases come from other tasks related to the VTT problem.
In the literature, authors have reported some automatic assessments, and the majority of them have come from the metrics used for information retrieval, machine translation, and image captioning tasks.
For retrieval-based methods, the most-reported measures in the literature are Recall at K and Mean Reciprocal Rank (MIR)~\citep{Craswell2009MeanRank}.
While for NLG-based methods, the state-of-the-art works report several $n$-gram-overlap-based metrics to automatically evaluate the quality of the output text (candidate) with the dataset's paired descriptions (references), being the most-reported metrics: 
\begin{itemize}
    \item \emph{BLEU} (Bilingual Evaluation Understudy~\citep{Papineni2002BLEU:Translation}, 2002), based on $n$-gram precision;
    \item \emph{ROUGE} (Recall Oriented Understudy of Gisting Evaluation~\citep{Lin2004Rouge:Summaries}, 2004), based on $n$-gram recall;
    \item \emph{METEOR} (Metric for Evaluation of Translation with Explicit Ordering~\citep{Banerjee2005METEOR:Judgments}, 2005), based on $n$-gram with synonym matching; and
    \item \emph{CIDEr} (Consensus-based Image Description Evaluation~\citep{Vedantam2015CIDEr:Evaluation}, 2015), based on precision and recall by \textit{TF-IDF} weighting of $n$-gram similarity.
\end{itemize}

A range of other automated metrics has been proposed for machine translation.
The explicit semantic match metrics define the similarity between human-written references and model generated candidate by extracting semantic information units from text beyond $n$-grams.
These metrics operate on semantic and conceptual levels and correlate well with human judgments~\citep{Celikyilmaz2020EvaluationSurvey}.
The \emph{SPICE} (Semantic Proportional Image Captioning Evaluation~\citep{Anderson2016SPICE:Evaluation}, 2015) metric has also been reported for video captioning.
This metric uses scene graphs to parse the candidate sentence to semantic tokens, such as object classes, relationship types, or attribute types.
% In this section, we cover these metrics and others less reported, but also suitable in the VTT problem.
In this section, we present the definition of these metrics and briefly discuss their advantages and limitations.
For more details on the evaluation of text generation models, we refer the reader to \citet{Celikyilmaz2020EvaluationSurvey}, a recent review on NLG evaluation methods. 


\subsection{Retrieval-specific Evaluation Metrics}

A standard evaluation metric for information retrieval methods is the \emph{Mean Inverted Rank (MIR)}~\citep{Craswell2009MeanRank}.
% This metric computes the average of the inverted ranks of results for a sample of queries.
It is a statistical measure that calculates the average over a set of $n$ queries.
Different scores are attributed inversely proportional to the rank of the first correct answer in the answer list.
\begin{equation}\label{ec:MIR}
\text{MIR} = \frac{1}{n}\sum_{i=1}^{n}\frac{1}{rank_{i}},
\end{equation}
\noindent where $rank_{i}$ is the rank position of the first correct answer of the $i$-th query.

$\text{MIR}$ has been used in the Matching \& Ranking subtask of the TRECVID challenge from 2017 but has not been frequently reported in the literature of video-text retrieval methods.
It is appropriate to evaluate models where there is only one relevant result or only cares about the highest-ranked one. 

In the context of recommendation systems, we are most likely interested in recommending top-$k$ items to the user.
So it makes more sense to compute \emph{precision} and \emph{recall} metrics in the first $k$ items instead of all the items.
Thus, in the context of VTT, the notion of precision and recall at $k$, where $k$ is a user-definable integer to match the top-$k$ recommended descriptions.
\emph{Recall at k (R@k)} is then the proportion of relevant descriptions found in the top-$k$ recommendations:
\begin{equation}
    % Recall@k = (# of recommended items @k that are relevant) / (total # of relevant items)
    \text{R@k} = \frac{r@k}{r},
\end{equation}
\noindent where $r@k$ is the number of recommended descriptions at $k$ that are relevant, and $r$ is the total number of relevant descriptions. 

Several state-of-the-art works report R@k results for some values of $k$, \eg R@1, R@5, R@10, R@50.
These works also report the \emph{mean average precision (mAP)} and \emph{median rank (MR)} scores.
The \emph{mAP} score considers whether all of the relevant items tend to get ranked highly.
Then, when there is only one relevant answer in the corpus, $\text{MIR}$ and $\text{mAP}$ are exactly equivalent under the standard definition of $\text{mAP}$.
For comparing methods performance, higher $\text{R@k}$ and $\text{mAP}$, and smaller $\text{MR}$ indicates better performance.
Usually, for evaluating the quality of learned joint embeddings, the authors also report these scores for the opposite problem: video retrieval from an input text.

% \textbf{Mean Inverted Rank (MIR)}~\citep{Craswell2009MeanRank} is common in information retrieval, and it is the average of the inverted ranks of results for a sample of queries. It is a statistical measure that calculates the average over a set of $n$ queries, where different scores are attributed inversely proportional to the rank of the first correct answer in the answer list.
% \begin{equation}\label{ec:MIR}
% MIR = \frac{1}{n}\sum_{i=1}^{n}\frac{1}{rank_{i}}
% \end{equation}
% \noindent in which $rank_{i}$ is the rank position of the first correct answer of the $i$-th query.


\subsection{Description Generation-specific Evaluation Metrics}

Early video description generation works~\citep{Guadarrama2013Youtube2text:Recognition, Krishnamoorthy2013GeneratingKnowledge, Rohrbach2013TranslatingDescriptions} used the \emph{SVO Accuracy} to measure whether the generated SVO triplets coheres with ground truth. 
This metric does not evaluate the quality of the generated sentence. 
% The purpose of this evaluation metric is to focus on the matching of broad semantics.
% Also, this metric ignores visual and language details. 
This evaluation metric aims to focus on the matching of general semantics and ignores visual and language details.

% In order to deal with this limitation, several $n$-gram-overlap-based metrics have been reporte

\textbf{Bilingual Evaluation Understudy computation (BLEU)}~\citep{Papineni2002BLEU:Translation} is based on the match between %\textit{uni}-gram (only one word) or 
$n$-grams (a sequence of $n$ words) of the candidate sequence and one or some reference sequences.
\emph{BLEU} is a weighted geometric mean of $n$-gram \emph{precision} scores, defined as:
\begin{equation*}
p_n = \frac{\sum_s \text{min}\big(c(s, \hat{y}), c(s, y)\big)}{\sum_s c(s, \hat{y})},
\end{equation*}
\noindent where $\hat{y}$ is the candidate sequence, $y$ is the reference sequence, $s$ is a $n$-gram sequence of $\hat{y}$, and $c(s, \hat{y})$ is the number of times that $s$ appears in $\hat{y}$.
The $\text{BLEU-N}$ metric is then:
\begin{equation}\label{eq:bleu}
    \log \text{BLEU-N} = \min(1-\frac{r}{c},0) + \sum_{n=1}^N w_n \log p_n,
\end{equation}
\noindent where $c$ and $r$ are the lengths of the candidate and reference sequences, respectively. %$p_n$ is the geometric average of the modified $n$-gram precisions, which is computed using $n$-grams up to length $N$. 
$N$ is the total number of $n$-gram precision scores to use, and $w_n$ %are positive weights summing to one.
is the weight for each precision score, which is often set to be $1/N$.

Equation \ref{eq:bleu} counts the position-independent matches among the candidate's $n$-grams and the reference's $n$-grams and computes the percent of matches (precision).
For video captioning, the most reported version is $\text{BLEU-4}$ with uniform weights $w_n = 1/N$. 
$\text{BLEU}$ was originally designed to evaluate long texts, and its use as an evaluation measure for individual sentences \textit{may not be fair}.

\textbf{Recall Oriented Understudy of Gisting Evaluation (ROUGE)}~\citep{Lin2004Rouge:Summaries} is a set of metrics designed for determining the quality of automatic summarization of long texts. 
Although mainly designed for evaluating summarization, it has also been widely used for evaluating short text production approaches, such as image captioning and video captioning.
It computes the $n$-gram \emph{recall} score of the candidate sentences with respect to those of reference~\citep{Lin2004Rouge:Summaries}. 
Similar to $\text{BLEU}$, it also is computed varying the number of $n$-grams. 
% Let $c_{match}(s)$ be the maximum number of co-occurrences of $n$-grams in the candidate sequences and a set of references $R$.
Let $c_{match}(s)$ be the number of times that the $n$-gram $s$ co-occur in the candidate sequence.
The $\text{ROUGE-N}$ score is then:
\begin{equation}
\text{ROUGE-N} = \frac{\sum_{y\in R}\sum_{s\in y}c_{match}(s)}{\sum_{y\in R}\sum_{s \in y}c(s)}
\end{equation}

% \begin{equation}
% \textrm{ROUGE-N} = \frac{\sum_{r\in R}\sum_{gram_n\ins}C_{match}(gram_n)}{\sum_{r\in R}\sum_{gram_n \in r}C(gram_n)}
% \end{equation}
\noindent where $s\in y$ is a $n$-gram sequence of the reference $y\in R$. 
The denominator $\sum_{y\in R}\sum_{s \in y}C(s)$ of the equation is the total sum of the number of $n$-grams occurring at the reference summary side.
Note that the number of $n$-grams in the denominator increases as more descriptions become available for reference.

In the same paper, the authors proposed several $\text{ROUGE-N}$ variants, such as  $\text{ROUGE-L}$, which is the most used variant for image and video captioning evaluation.
For $\text{ROUGE-L}$, the longest common subsequence (LCS)-based \emph{F-measure} is computed to estimate the similarity between the candidate sentence and the reference.
In other words, it measures the longest matching sequence of words using LCS. 
One advantage of using LCS is that it does not require consecutive matches, but it requires in-sequence matches that indicate sentence-level word order~\citep{Lin2004Rouge:Summaries}. 
The other advantage is that the $n$-gram length does not need to be predefined since ROUGE-L automatically includes the longest common $n$-grams shared by the reference and candidate text.

Formally, given two sequences $\hat{y}$ and $y$, the $\text{LCS}(\hat{y}, y)$ the length of the LCS of $\hat{y}$ and $y$.
Let $m$ the length of $\hat{y}$ and let $n$ the length of $y$.
The LCS-based \emph{F-measure} is then:
\begin{equation}
    \begin{split}
        R_{lcs} &= \frac{\text{LCS}(\hat{y}, y)}{m},\\
        P_{lcs} &= \frac{\text{LCS}(\hat{y}, y)}{n},\\
        F_{lcs} &= \frac{(1+\beta^2)R_{lcs}P_{lcs}}{R_{lcs}+\beta^2P_{lcs}},       
    \end{split}
\end{equation}
\noindent where $\beta=\frac{P_{lcs}}{R_{lcs}}$ when $\frac{\partial F_{lcs}}{\partial P_{lcs}}=\frac{\partial F_{lcs}}{\partial R_{lcs}}$.
Notice that $\text{ROUGE-L}$ is one when $\hat{y} = y$ since $\text{LCS}(\hat{y}, y) = m$ or $n$; while $\text{ROUGE-L}$ is zero when $\text{LCS}(\hat{y}, y) = 0$, \ie there is nothing in common between $\hat{y}$ and $y$.

Another metric that has been widely used for evaluating image and video captioning models is the \textbf{Metric for Evaluation of Translation with Explicit Ordering (METEOR)}~\citep{Banerjee2005METEOR:Judgments}.
Compared to BLEU (based on precision only), METEOR is based on the harmonic mean of the \textit{uni}-gram precision and recall, in which recall is weighted higher than precision~\citep{Celikyilmaz2020EvaluationSurvey}.
This metric couples BLEU scores $\forall n\in\{1,2,3,4\}$ into a single performance value, and it was designed to improve correlation with human judgments.
Some variants of this metric also introduce the semantic match for addressing the reference-translation variability problem.
These variants allow morphological variation, synonyms, stems, and paraphrases to be recognized as valid translations.

The classic version of the METEOR score between a candidate translation and a reference translation is defined as follows.
% In the case of multiple sentences of reference, the maximum between the candidate and each reference is considered.
% The score is computed as follow: 
First, the $uni$-gram precision $P$ and recall $R$ are respectively calculated by:
\begin{equation}\label{eq:precision-recall}
\begin{split}
    P=&\frac{u}{u_c}, \text{ and} \\
    R=&\frac{u}{u_r},
\end{split}
\end{equation}
\noindent where $u$ is the number of $uni$-grams in the candidate translation that also appear in the reference translation, $u_c$ is the number of $uni$-grams in the candidate translation, and $u_r$ is the number of $uni$-grams in the reference translation.

Next, the $F_{mean}$ is computed by combining the precision and recall (defined in Equation~\ref{eq:precision-recall}) via a parameterized harmonic mean~\citep{Rijsbergen1979InformationRetrieval}: %that places most of the weight on recall.
\begin{equation}\label{eq:f-mean}
    F_{mean}=\frac{P \times R}{\alpha \times P + (1-\alpha) \times R},
\end{equation}
% where is common to use $\alpha=10$ they used a harmonic-mean of $P$ and $9R$, resulting formula:

% \begin{equation}\label{eq:f-mean}
%     F_{mean}=\frac{10PR}{R+9P}
% \end{equation}

% Before METEOR, the metrics only account for congruity with respect to single words but not with respect to larger segments that appear in both the reference and the candidate sentence.
% To take them into account, longer $n$-gram matches are used to compute a penalty $p$ for the alignment, grouping $uni$-grams into the fewest possible chunks, where a chunk is defined as a set of $uni$-grams that are adjacent in the candidate and reference.
To account for gaps and differences in word order, METEOR calculates a fragmentation penalty.
This calculation uses the total number of matched \textit{uni}-grams $u$ (averaged over candidate and reference) and the number of chunks $ch$, where a chunk is defined as a set of adjacent \textit{uni}-grams in the candidate and reference.
%The longer the adjacent mappings between the candidate and the reference, the fewer chunks there are. A translation that is identical to the reference will give just one chunk. 
The penalty $p$ is then computed by:
\begin{equation}
    p=\gamma\left(\frac {ch}{u}\right)^\beta,
\end{equation}
% \begin{equation}
%     p=0.5\left(\frac {c}{u_m}\right)^3,
% \end{equation}
\noindent where $\gamma$ determines the maximum penalty ($0 \leq \gamma \leq 1$), and $\beta$ determines the functional relation between the fragmentation and the penalty.
% The penalty has the effect of reducing the $F_{mean}$ (defined in (\ref{eq:f-mean})) by up to $50\%$ if there are no $bi$-gram or longer matches.
The penalty has the effect of reducing the $F_{mean}$ (defined in Equation~\ref{eq:f-mean}) if there are no $bi$-grams or longer matches.

The final METEOR score is then calculated by:
\begin{equation}\label{eq:meteor}
    \text{METEOR}=F_{mean}\times(1-p)    
\end{equation}

% To calculate a score over a whole corpus, or collection of segments, the aggregate values for $P$, $R$ and $p$ are taken and then combined using the same formula.

Another metrics that also considers both precision and recall is \textbf{Consensus-based Image Description Evaluation (CIDEr)} considers.
CIDEr was originally proposed for image captioning by \citet{Vedantam2015CIDEr:Evaluation} and is based on the consensus protocol and the average cosine similarity between $n$-grams in the candidate caption and the reference captions.

Intuitively, CIDEr measures how often $n$-grams in the candidate caption are present in the reference captions. 
For this, CIDEr assumes that $n$-grams that do not appear in the reference captions should not be in the candidate sentence.
While $n$-grams that commonly occur across the corpus should be given lower weights, they are likely to be less informative. 
Given these assumptions, a \emph{Term Frequency Inverse Document Frequency (TF-IDF)} weight is calculated for each $n$-gram.

Given the $i$-th input video $x_i$, the set of reference captions $Y_i = \{y_{i1}, \ldots, y_{im}\}$ and a candidate caption $\hat{y}$, all words in both candidate and references are first mapped to their stem or root forms.
For example, ``generates'', ``generation'', ``generated'' and ``generating'' are all reduced to ``generate''. 
Then, the TF-IDF weighting $g_k(y_{ij})$ for $k$-th $n$-gram $\omega_k$ and the $y_{ij}$ reference caption is performed by:
\begin{equation}
    g_k(y_{ij}) = \frac{h_k(y_{ij})}{\sum_{\omega_l\in\Omega}h_l(y_{ij})}\log \Big(\frac{|V|}{\sum_{x_p\in V}\min(1, \sum_q h_k(y_{pq}))}\Big),
\end{equation}

\noindent where $h_k(y_{ij})$ represents the number of times that the $n$-gram $\omega_k$ occurs in the reference caption $y_{ij}$, $\Omega$ is the vocabulary of all $n$-grams, and $V$ is the set of all videos in the dataset.

The average cosine similarity between them calculates the $\text{CIDEr}_n$ score for a particular $n$-gram between the candidate caption $\hat{y}_i$ and the reference captions $Y_i$: 
% The $\text{CIDEr}_n$ score for a particular $n$-gram between the candidate caption $\hat{y}_i$ and the reference captions $Y_i$, is calculated by the average cosine similarity between them:
\begin{equation}\label{eq:cider_n}
    \text{CIDEr}_n(\hat{y}_i, Y_i) = \frac{1}{m}\sum_j\frac{\textbf{g}^n(\hat{y}_i) \times \textbf{g}^n(y_{ij})}{\norm[1]{\textbf{g}^n(\hat{y}_i)}\norm[1]{\textbf{g}^n(y_{ij})}},
\end{equation}

\noindent where $\textbf{g}^n(\hat{y}_i)$ is a vector formed by the $g_k(\hat{y}_i)$ weights and $\textbf{g}^n(y_{ij})$ is a vector formed by $g_k(\hat{y}_i)$ weights, corresponding to all $n$-grams of length $n$ of the candidate $\hat{y}_i$ and the references $y_{ij}$, respectively. 
$\norm[1]{\textbf{g}^n(\hat{y}_i)}$ and $\norm[1]{\textbf{g}^n(y_{ij})}$ are the magnitudes of these vectors.

To capture richer semantics and grammatical properties, the authors proposed to compute a higher-order (longer) $n$-grams.
They combined the scores from $n$-grams varying lengths as follows:
\begin{equation}
    \text{CIDEr}(\hat{y}_i, Y_i)=\sum_{n=1}^N w_n \text{CIDEr}_n(\hat{y}_i, Y_i)
\end{equation}
\noindent Here, the authors found that uniform weights $w_n=1/N$ and $N=4$ work the best, empirically.
Likewise, for benchmark evaluation on image and video captioning, the most popular version of this metric, $\text{CIDEr-D}$~\citep{Vedantam2015CIDEr:Evaluation, Chen2015MicrosoftServer}, is used.
$\text{CIDEr-D}$, among other modifications, prevents higher scores for descriptions that erroneously fail for human judgments. CIDEr-D does this, by clipping, for a specific n-gram, the number of candidate occurrences to the number of reference occurrences.
These modifications result in the following version of Equation~\ref{eq:cider_n}:
\begin{equation}\label{eq:ciderd_n}
    \text{CIDEr-D}_n(\hat{y}_i, Y_i) = \frac{10}{m}\sum_j \Bigg(\exp \bigg(\frac{-l(\hat{y}_i)-l(y_{ij})^2}{2\sigma^2}\bigg) \times \frac{\min(\textbf{g}^n(\hat{y}_i), \textbf{g}^n(y_{ij})) \cdot \textbf{g}^n(y_{ij})}{\norm[1]{\textbf{g}^n(\hat{y}_i)}\norm[1]{\textbf{g}^n(y_{ij})}}\Bigg),
\end{equation}
\noindent where $l(\hat{y}_i)$ and $l(y_{ij})$ denote the lengths of candidate and reference sentences respectively, and $\sigma = 6$ is usually used.
This penalty and the factor ten produce that, unlike other metrics, the scores can be higher than one but lower than ten.

% \subsubsection{Other Reported Metrics}

% \item[WMD, 2015:] Word Mover's Distance measures the dissimilarity between two text documents as the minimum distance that the embedded words of one document need to ``travel'' to reach the embedded words of another document~\citep{Kusner2015FromDistances}. 
% Firstly, the descriptions are transformed into normalized \emph{bag-of-words} vectors (\emph{nBOW}).
% Compared to BLEU, ROUGE, and CIDEr, it is lower affected by the words order or the exchange of synonyms.
% Although similar to CIDEr and METEOR, it gets a high correlation against human judgments.

\subsubsection{Explicit Semantic Match-based Metrics}

Beyond $n$-grams, the semantic content matching metrics measure the similarity between the generated caption and the reference captions in the dataset by extracting explicit semantic information units.
These metrics have shown well-correlation with human judgments.

The \textbf{Semantic Proportional Image Captioning Evaluation (SPICE)}\label{metric:spice} metric~\citep{Anderson2016SPICE:Evaluation} is based on tuples of scene graphs of the generated candidate description and all reference descriptions. 
These scene graphs encode the related video in a skeleton form, parsing the descriptions using two stages: (1) syntactic dependencies extraction and (2) a rule-based graph mapping.
This skeleton represents the texts as semantic tokens, such as object classes, relationship types, or attribute types. 
After a proper parsing, SPICE then computes the \emph{F-SCORE} using the candidate and reference scene graphs over the conjunction of logical tuples representing semantic propositions in the scene graph.
% the descriptions are generated using all combinations of objects of the graph (a tuple of graphs).
% Then, the \emph{F-score} between the candidate-reference tuples is computed. 

Better than improved versions of METEOR and CIDEr, SPICE also uses synonyms match by the encoding into semantic scene graphs.
However, one limitation (not widely reported) of this metric is its dependency on the parsing quality.
Another major limitation is that even though SPICE correlates well with human evaluations, it ignores the generated captions' fluency~\citep{Celikyilmaz2020EvaluationSurvey, Sharif2018Learning-basedEvaluation}.

\textbf{Semantic Text Similarity (STS)} was introduced in the TREC\-VID 2016 as an experimental semantic similarity metric~\citep{Han2013UMBC_EBIQUITY-CORE:Systems}, and it has been used in this competition~\citep{Awad2016TRECVIDHyperlinking, Awad2017TrecvidHyperlinking, Awad2018TRECVIDSearch, Awad2019TRECVIDRetrieval, Awad2020TRECVIDDomains}, in addition to BLEU, METEOR, and CIDEr metrics.
This metric measures how semantically similar is the submitted description to the ground-truth description.
It is based on distributional similarity, and Latent Semantic Analysis (LSA) complemented with semantic relations extracted from WordNet.


\subsubsection{Limitations}\label{sec:eval-limitations}
Most video captioning metrics have been adopted from machine translation or image captioning and do not well-measure the quality of the generated descriptions from videos.
Automated metrics should agree well with human judgment to be useful in practice.
In this sense, BLEU and ROUGE are not optimal~\citep{Reiter2018ABLEU, Schluter2017TheROUGE} and have been shown to correlate with humans weakly~\citep{Vedantam2015CIDEr:Evaluation, Hodosh2015FramingAbstract}. 
In contrast, the METEOR and CIDEr metrics have shown a better correlation with humans when judging the overall quality of language descriptions for image and video captioning tasks.
Specifically, CIDEr shows a high agreement with consensus as assessed by humans~\citep{Vedantam2015CIDEr:Evaluation}.
Simultaneously, METEOR addresses the problem of reference description variability, allowing the recognition of morphological variants and synonyms as adequate descriptions.

Due to this discrepancy between metrics, the automatic evaluation is often accompanied by human evaluators accessing the candidate texts for their intrinsic qualities (\eg correctness, fluency, factuality, and discourse coherency and consistency)~\citep{Celikyilmaz2020EvaluationSurvey} and human preferences.
Human evaluations have several challenges.
They are expensive, time-consuming and the people who are going to evaluate will require extensive domain expertise.
To ease this process, some crowd-sourcing platforms like Amazon Mechanical Turk (AMT) exist.
We can post the method's outputs with a detailed description of how people must evaluate, and we get our results based on convinced voting.
However, that also has downsides, such as checking evaluations and evaluators' consistency and quality without knowing them.

In the VTT task of the TRECVID Challenge (see Section~\ref{sec:challenge:trecvid}), the organizers address this limitation by evaluating the automatic video descriptions with the \emph{Direct Assessment (DA)} method~\citep{Awad2020TRECVIDDomains} in addition to standard metrics.
DA is an accurate method proposed by \cite{Graham2018EvaluationAssessment} to control crowd-sourcing quality, which is efficient and cost-effective for tuning automatic evaluation metrics.
They addressed the limitations of crowd-sourced judgments by automatically modifying candidate captions and degrading their quality, and examining how human judges rated the degraded captions.
They demonstrated that this process is ten times more effective at finding significant differences between competing systems than previous methodologies.
Furthermore, the use of DA for evaluating the variable number of annual participants in the TRECVID-VTT task has shown its scalability, robustness, and replicability.


% At the same time, some authors noted that the performance of metrics is correlated with the number of descriptions associated with each video in the datasets.
% In this sense, some of the datasets have a few numbers of descriptions per video; for example, M-VAD~\citep{Torabi2015UsingResearch} and MPII-MD~\citep{Rohrbach2015ADescription, Rohrbach2017GeneratingPeople} have one only description per video. And~\citet{Vedantam2015CIDEr:Evaluation} found that five sentences are not sufficient for measuring how a ``majority'' of humans would describe an image.
% Also, they found that, except BLEU computed on \textit{uni}-grams, one way to improve most metrics is by increasing the number of reference sentences, which is an indicator of their poor power. 
% Moreover, collecting a large number of references can be very time-consuming, expensive, and difficult for less common languages.

%Finally,~\citet{Hodosh2015FramingAbstract} indicated that BLEU and ROUGE are not useful metrics for this task. BLEU in particular failed to reveal statistically significant differences between systems that the “experts” identified.

==> sections/loss-functions.tex <==
\section{Loss Functions for Optimization}\label{sec:loss}

In previous sections, we studied the state-of-the-art techniques for creating effective VTT methods.
However, we have not detailed how these models are trained.
This section analyzes the different objective functions for video captioning methods in Section~\ref{sec:loss-dg} and video description retrieval methods in Section~\ref{sec:loss-mr}. 
In particular, in Section~\ref{sec:loss-dg}, we include an analysis of sequence level- and reinforcement learning-based strategies.

\subsection{For Description/Caption Generation Methods}\label{sec:loss-dg}
After predicting the probability distribution of each word in the vocabulary by Equation~\ref{eq:prob}, 
most video-captioning models are trained by the %principle of Maximum Likelihood Estimation (Cross-Entropy minimization, CELoss).
cross-entropy loss minimization (CELoss).
With $\text{CELoss}$, the model is trained to %maximize the conditional log-likelihood of 
be good at greedily predicting the next correct word of the reference caption.
Given a target caption, $\hat{y}~=~(\hat{w}_1, \hat{w}_2, \dots, \hat{w}_L)$ describing an input video, one minimizes:
\begin{equation}
    \mathcal{L}_\Theta = -\sum_{t=1}^L \log \text{p}_\Theta(\hat{w}_t|\hat{w}_{<t}),
\end{equation}

% \begin{equation}
%     \log \text{p}_\Theta(y|x) = \sum_{t=1}^T \text{p}_\Theta(w_t|w_{<t}),
% \end{equation}

% \noindent where $\Theta$ are all the learnable parameters of the captioning model, $w_t$ is the $t$-th generated word, $w_{<t}$ is the previously generated $t-1$ words, and $T$ denotes the number of words in the sentence.

\noindent where $\Theta$ are all the learnable parameters of the captioning model, $\hat{w}_t$ is the $t$-th word in the ground-truth caption, and $\hat{w}_{<t}$ are the first $t-1$ words in the ground-truth caption. %, and $L$ denotes the number of words in the sentence.
$\text{p}_\Theta(\hat{w}_t|\hat{w}_{<t})$ is modeled by a logistic function as the \emph{decoder} network's output layer, understood as the probability distribution of words in the vocabulary.

However, at test time, the model has only access to its predictions, which may not be correct.
Additionally, video captioning's popular evaluation metrics are based on $n$-gram overlapping between the generation and reference captions, \eg BLEU~\citep{Papineni2002BLEU:Translation}.
This discrepancy leads to a problem called \textit{exposure bias}~\citep{Ranzato2016SequenceNetworks} in sequential decoders.
Due to this discrepancy, the word-level $\text{CELoss}$ function is not directly related to the most used evaluation metrics for video captioning~\citep{Ranzato2016SequenceNetworks, Pasunuru2017ReinforcedRewards}. %, which are sentence-level metrics. 
Some state-of-the-art works show that conventional $\text{CELoss}$ cannot extract the effectiveness of their models.

% most video-captioning models are trained by the principle of Maximum Likelihood Estimation (MLE), also known as Cross-Entropy minimization ($\text{CELoss}$)~\citep{Goodfellow2016DeepLearning}.
% With $\text{CELoss}$, the model is trained to maximize the probability of generating the next correct word of the reference caption:
% \begin{equation}
%     \text{CELoss}_\Theta = -\sum_{t=1}^T \log P(\hat{y}_t|\hat{y}_{<t}),
% \end{equation}

% \noindent where $\Theta$ are all the learnable parameters of the captioning model, $\hat{y}_t$ is the $t$-th word in the ground-truth caption, $\hat{y}_{<t}$ are the first $t-1$ words in the ground-truth caption, and $T$ denotes the number of words in the sentence.

% However, at test time, the model has only access to its predictions, which may not be correct.
% Additionally, the popular evaluation metrics used for video captioning are based on n-gram overlapping between the generation and reference captions, \eg BLEU~\citep{Papineni2002BLEU:Translation}.
% This discrepancy leads to a problem called \textit{exposure bias}~\citep{Ranzato2016SequenceNetworks} in sequential decoders.
% For this discrepancy, the word-level $\text{CELoss}$ function is not directly related to the most used evaluation metrics for video captioning~\citep{Ranzato2016SequenceNetworks, Pasunuru2017ReinforcedRewards}, which are sentence-level metrics. 
% Some state-of-the-art works show that conventional $\text{CELoss}$ cannot extract the effectiveness of their models.

To overcome this limitation while operating with explicit supervision at the sequence level, \citet{Chen2020ASampling} proposed a loss function that weights the $\text{CELoss}$ according to the length of the reference captions. %makes the forward of the model generates a high loss when the ground-truth captions are very long.
% Given a ground truth caption, $y~=~\{w_1, w_2, \dots, w_L\}$ describing an input video, they minimize:
\begin{equation}
    \mathcal{L}_\Theta' = -\frac{1}{L^\beta}\sum_{t=1}^{L}\log \text{p}_\Theta(\hat{w}_t|\hat{w}_{<t}),
\end{equation}
% \begin{equation}
%     L_\Theta = -\frac{1}{L^\beta}\sum_{t=1}^{L-1}\log p_\theta(w_t|w_{<t}),
% \end{equation}

\noindent $L$ is the length of the ground-truth caption, and $\beta \in [0,1]$ is a hyperparameter of the model. 
%Therefore, training the model with this loss function implies that generated sentences are more concise. In contrast, if $\beta=1$ the loss is the same as $\text{CELoss}$.
The hyperparameter $\beta \in [0,1]$ regulates the length of the generated sentences.
The higher the value of $\beta$, the lower the loss produced by the function, and vice versa.
Thus, a value of $\beta$ near 0 implies that the model rapidly adapts to generate concise sentences that could affect their syntactic correctness.

Another strategy to overcome this limitation is to expose the model to its own predictions rather than just the training data, and directly optimize the task-specific evaluation metric.
The models trained following this strategy commonly use policy gradients and mixed-loss methods for \emph{reinforcement learning}~\citep{Pasunuru2017ReinforcedRewards}.
Instead of maximizing the likelihood of prediction at each step, the model first generates the whole sequence.
A reward (often one of the evaluation metrics at test time, \eg CIDEr) is estimated by comparing the output text to the ground-truth description.
The reward is then used to update the model parameters, learning to maximize the evaluation metric during training.

In particular, state-of-the-art methods based on reinforcement learning use a standard algorithm called \emph{policy learning}, which allows us to maximize a non-differentiable reward efficiently.
These methods view the description generation model as an \emph{agent} that interacts with an \emph{environment} with access to reference texts.
Each input video represents a \emph{state}, and each \emph{action} is an output text generated by the agent.
The agent predicts an output caption $\hat{y}$ using \emph{policy} $p(\hat{y}|x, \Theta)$, where $x$ is the input video and $\Theta$ are model parameters.
After each action, the agent receives an immediate \emph{reward} corresponding with how well the final caption resembles the reference text.
The transition between states is trivial because the inputs are interdependent.
The models learn to optimize the policy such that the agent can take an optimal action optimizing its reward given a state.

The reward function plays a crucial role here, which is defined such as that it captures the critical aspects of the target output concerning the benchmark dataset.
Several methods~\citep{Chen2018LessCaptioning, Li2019End-to-EndLearning, Pasunuru2017ReinforcedRewards, Phan2017Consensus-basedCaptioning, Wang2018VideoLearning, Wang2019ControllableNetwork} use the CIDEr score as the reward over the MSVD and MSR-VTT datasets.
In particular, \citet{Pasunuru2017ReinforcedRewards} proposed  CIDEnt-RL, which penalizes the phrase-matching metric (CIDEr) based reward when the entailment score is low.
While \citet{Phan2017Consensus-basedCaptioning} compared the performance using different metrics as a reward, \ie BLEU-4, METEOR, ROUGE$_L$, and CIDEr.
Although the improvement on different metrics is unbalanced because the improvements on other metrics are not as large as the specific metric directly optimized, they obtain the best performance for all metrics optimizing the CIDEr score.

\subsection{For Matching \& Ranking Methods}\label{sec:loss-mr}
As we explained in Section~\ref{sec:matching-ranking}, recent methods for matching \& ranking video descriptions use two encoders $f(\cdot)\in \mathbb{R}^d$ and $g(\cdot)\in \mathbb{R}^d$ for mapping the videos and captions into a joint space, respectively.
After defining these mapping functions' structure, we need to determine how to train them to obtain accurate representations that capture both modalities' relationship.
The \emph{triplet-ranking-loss} function is a standard margin-based loss for training retrieval models.
Motivated on the nearest-neighbor classification technique~\citep{Weinberger2005DistanceClassification}, \citet{Schroff2015FaceNet:Clustering} proposed this loss function for the Face Recognition problem~\citep{Parkhi2015DeepRecognition}.

Let $(x,y)\in \mathcal{D}$ a video-description pair of the dataset and assume that $y^\star$ is an arbitrary description in the dataset not associated with $x$ (a negative example).
Their projections in the joint space are $f(x) = z_x$, $g(y) = z_y$, and $g(y^\star) = z_{y^\star}$.
Assume $\text{dist}(\cdot,\cdot)$ is a distance function in $\mathbb{R}^d$.
This loss function tries to ensure that the distance between the anchor $z_x$ and positive encoding $z_y$ is less than the distance between the anchor and any negative encoding. 
We would like the following to hold:
% Given the encoding of an anchor video $f(v^a) = x^a$, the encoding of their positive captions $g(s^p) = y^p$, and the encoding of any arbitrary caption $g(s^n) = y^n$ in the dataset not associated with $v^a$ (a negative example). 
% This loss function tries to ensure that the distance between the anchor and positive encoding is less than the distance between the anchor and any negative encoding. 
% Assume $\text{dist}(\cdot,\cdot)$ is a distance function in $\mathbb{R}^d$.
% We would like the following to hold:
\begin{equation}
    dist(z_x, z_y) + \alpha < dist(z_x, z_{y^\star}),
\end{equation}
\noindent where $\alpha$ is a margin that is enforced between positive and negative pairs.
% \begin{equation}
%     dist(x^a, y^p) + \alpha < dist(x^a, y^n), \forall (x^a, y^p, y^n) \in \mathcal{T},
% \end{equation}
% $\alpha$ is a margin hyperparameter that is enforced between positive and negative pairs, and $\mathcal{T}$ is the set of all possible triplets of anchor, positive and negative, in the training set.
This gives  rise  to  a  natural  optimization problem in which one wants to minimize:
\begin{equation}
    L_\Theta = \max\bigg\{\, 0,\; \text{dist}\big(z_x,\,z_y\big) + \alpha - \text{dist}\big(z_x,\,z_{y^\star}\big)\bigg\}
\end{equation}
% \begin{equation}
%     L_\Theta = \max\bigg\{\, 0,\; \text{dist}\big(x^a,\,y^p\big) + \alpha - \text{dist}\big(x^a,\,y^n\big)\bigg\}
% \end{equation}

% \begin{equation}
%     L_\Theta = -\max(D_\Theta(x_i^a, x_i^n) - D_\Theta(x_i^a, x_i^p) + \alpha, 0),
% \end{equation}

% \noindent where $N$ is the number of triplets in each mini-batch.

This formulation is the classic version of triple-ranking loss and is used in many different applications with the same formulation or minor variations. However, in the literature, it can be found under other names such as ranking loss, margin loss, contrastive loss, triplet loss, and hinge loss, which can be confusing.
For VTT, researchers have adapted several distance functions and triplets selection approaches.
For example, \citet{Dong2019DualRetrieval} proposed to use the improved marginal ranking loss~\citep{Faghri2018VSE++:Negatives}, which penalizes the model taking into account the hardest negative examples.
In this improved version, one considers a tuple 
$(x,y,x^\star,y^\star)$ where $(x,y)\in \mathcal{D}$, $y^\star$ is the closest negative example for $x$, and $x^\star$ is the closest negative example for $y$.
Their projections in the joint space are $f(x) = z_x$, $g(y) = z_y$, $f(x^\star) = z_{x^\star}$, and $g(y^\star) = z_{y^\star}$.
% $(x^a,y^p,x^\star,y^\star)$ where $(x^a,y^p)\in \mathcal{D}$, $y^\star$ is the closest negative example for $x^a$, and $x^\star$ is the closest negative example for $y^p$.
They trained the model attending to the loss function:
% \begin{equation}
% \begin{split}
%     L_\Theta = 
%     \max\bigg\{\, 0,\; \text{dist}\big(x^a,\,y^p\big) + \alpha - \text{dist}\big(x^a,\,y^\star\big)\bigg\} + 
%     \max\bigg\{\, 0,\; \text{dist}\big(x^a,\,y^p\big) + \alpha - \text{dist}\big(x^\star,\,y^p\big)\bigg\}
% \end{split}
% \end{equation}
\begin{equation}\label{eq:loss:improved-triplet-loss}
\begin{split}
    L_\Theta' = &\max\bigg\{\, 0,\; \text{dist}\big(z_x,\,z_y\big) + \alpha - \text{dist}\big(z_x,\,z_{y^\star}\big)\bigg\} \\
                & + \max\bigg\{\, 0,\; \text{dist}\big(z_x,\,z_y\big) + \alpha - \text{dist}\big(z_{x^\star},\,z_y\big)\bigg\}
\end{split}
\end{equation}
\noindent where the distance function $\text{dist}(\cdot,\cdot)$ they used was the cosine distance function.

% \begin{equation}
% \begin{split}
%     L_\Theta = -\frac{1}{N}\sum_{i=1}^{N} (\max(D_\Theta(x_i^a, x_i^n) - D_\Theta(x_i^a, x_i^p) + \alpha, 0) + \max(D_\Theta(x_i^b, x_i^p) - D_\Theta(x_i^a, x_i^p) + \alpha, 0)),
% \end{split}
% \end{equation}

% \noindent where $x_i^b$ and $x_i^n$ represent a negative video sample 's encoding for the caption $s_i^p$ and a negative caption's encoding for video $v_i^a$, respectively. 
% However, they do not sample them randomly. They choose the most similar yet negative encoded caption and video in each mini-batch. 

Recently, \citet{Ging2020COOT:Learning} have proposed another form of training their cooperative hierarchical models.
In the context of video-paragraph datasets, they introduced a \emph{cross-modal cycle-consistency loss} to enforce the semantic alignment between clips and sentences.
The cycle-consistency uses transitivity as an objective for training~\citep{Chen2019Cycle-ConsistencyAnswering, Dwibedi2019TemporalLearning, Wang2019LearningTime, Zhu2017UnpairedNetworks}, and it has been used for tasks like temporal video alignment~\citep{Dwibedi2019TemporalLearning} and visual question answering~\citep{Chen2019Cycle-ConsistencyAnswering}.
In contrast to previous models~\citep{Dwibedi2019TemporalLearning} that only work on the video domain, \citet{Ging2020COOT:Learning} aligned video and text in a cross-modal way.
They defined the cyclical structure as follows.

Given a sequence of video clip embeddings $Z_x=\{z_{x1}, \ldots, z_{xn}\}$ of an input video $x$ and sentence embeddings $Z_y=\{z_{y1}, \ldots, z_{ym}\}$ of the reference paragraph $y$.
We first find the soft nearest neighbor~\citep{Dwibedi2019TemporalLearning} of each sentence embedding $z_{yi}$ in the clip sequence by:
\begin{equation}
    \hat{z_x} = \sum_{j=1}^n \alpha_j z_{xj},
\end{equation}
\noindent where $\alpha_j$ represents the similarity score of clip embedding $z_{xj}$ to sentence embedding $z_{yi}$, computed by:
\[
\alpha_j = \frac{\exp(-\norm[1]{z_{yi}-z_{xj}}^2)}{\sum_{k=1}^n\exp(-\norm[1]{z_{yi}-z_{xk}}^2)}
\]

\noindent We then cycle back from $\hat{z_x}$ to the sentences embeddings sequence $Z_y$ and calculate the soft location by:
\begin{equation}
    \hat{i} = \sum_{j=1}^m \beta_j j,
\end{equation}
\noindent where $\beta_j$ represents the similarity score of sentence embedding $z_{yj}$ to the soft clip embedding $\hat{z}_{x}$, computed by:
\[
\beta_j = \frac{\exp(-\norm[1]{\hat{z}_x-z_{yj}}^2)}{\sum_{k=1}^n\exp(-\norm[1]{\hat{z}_{x}-z_{yk}}^2)}
\]

Given these to locations $i$ and $\hat{i}$ in the sequence of sentence embeddings $Z_y$, we assume that the embedding $z_{yi}$ is semantically cycle-consistent if and only if it cycles back to the original location, \ie $i = \hat{i}$.
This loss aims to penalize deviations from cycle-consistency for sampled sets of clips and sentences, which encourages semantic alignment between vision and text representations in the joint embedding space.
The objective is then, the distance between the source index $i$ and the soft destination index $\hat{i}$:
\begin{equation}
    \mathcal{L}_{CMC} = \norm[2]{i-\hat{i}}^2
\end{equation}

For the final loss of the model, the authors combined $\mathcal{L}_{CMC}$ with four other losses.
Three of these losses are based on ranking losses (Equation~\ref{eq:loss:improved-triplet-loss}) obtained from clip-sentence level, video-paragraph level, and global context level.
The other one, proposed by \citet{Zhang2018Cross-ModalText}, models the clustering of low-level and high-level semantics in the joint embedding space:
\begin{equation}
    \mathcal{L}_{cluster} = \mathcal{L}_{low} + \mathcal{L}_{high}
\end{equation}

\noindent Here, the $\mathcal{L}_{low}$ part models the low-level semantics clustering by the sum of $L_\Theta'$ (defined in Equation~\ref{eq:loss:improved-triplet-loss}) for all tuples $(z_{xi}, z_{yi}, z_{x'j}, z_{y'j})$ such that $(x', y')\in\mathcal{D}$ and $x' \neq x$.
So, $z_{x'j}$ and $z_{y'j}$ are clip-sentence-level intra-modality negative examples such that $z_{x'j}$ is a negative example for $z_{xi}$ computed by the video encoder $f(\cdot)$, and $z_{y'j}$ is a negative example for $z_{yi}$ computed by the text encoder $g(\cdot)$.
\[
\begin{split}
\mathcal{L}_{low} = \sum_i \sum_{j, (x', y')\in \mathcal{D}, x' \neq x} \Bigg( 
&\max\bigg\{\, 0,\; \text{dist}\big(z_{xi},\,z_{yi}\big) + \gamma - \text{dist}\big(z_{xi},\,z_{x'j}\big)\bigg\} \\
&+ \max\bigg\{\, 0,\; \text{dist}\big(z_{xi},\,z_{yi}\big) + \gamma - \text{dist}\big(z_{y'j},\,z_{yi}\big)\bigg\} \Bigg),
\end{split}
\]
\noindent where $\gamma$ is a constant margin.

The $\mathcal{L}_{high}$ part captures the high-level semantics clustering by the sum of $L_\Theta'$ (defined in Equation~\ref{eq:loss:improved-triplet-loss}) for all tuples $(z_x, z_y, z_{x'}, z_{y'})$ such that $(x', y')\in\mathcal{D}$ and $x' \neq x$.
So, $z_{x'}$ and $z_{y'}$ are video-paragraph-level intra-modality negative examples such that $z_{x}$ is a negative example for $z_{x}$ computed by the video encoder $f(\cdot)$, and $z_{y'}$ is a negative example for $z_{y}$ computed by the text encoder $g(\cdot)$.
\[
\begin{split}
\mathcal{L}_{high} = \sum_i \sum_{(x', y')\in \mathcal{D}, x' \neq x} \Bigg( 
&\max\bigg\{\, 0,\; \text{dist}\big(z_x,\,z_y\big) + \rho - \text{dist}\big(z_x,\,z_{x'}\big)\bigg\} \\
&+ \max\bigg\{\, 0,\; \text{dist}\big(z_x,\,z_y\big) + \rho - \text{dist}\big(z_{y'},\,z_y\big)\bigg\} \Bigg),
\end{split}
\]
\noindent where $\rho$ is a constant margin.
